Understanding the Design-Space of Sparse/Dense Multiphase GNN dataflows on Spatial Accelerators

Graph Neural Networks (GNNs) have garnered a lot of recent interest because of their success in learning representations from graph-structured data across several critical applications in cloud and HPC. Owing to their unique compute and memory characteristics that come from an interplay between dense and sparse phases of computations, the emergence of reconfigurable dataflow (aka spatial) accelerators offers promise for acceleration by mapping optimized dataflows (i.e., computation order and parallelism) for both phases. The goal of this work is to characterize and understand the design-space of dataflow choices for running GNNs on spatial accelerators in order for mappers or design-space exploration tools to optimize the dataflow based on the workload. Specifically, we propose a taxonomy to describe all possible choices for mapping the dense and sparse phases of GNN inference, spatially and temporally over a spatial accelerator, capturing both the intra-phase dataflow and the inter-phase (pipelined) dataflow. Using this taxonomy, we do deep-dives into the cost and benefits of several dataflows and perform case studies on implications of hardware parameters for dataflows and value of flexibility to support pipelined execution.

==> 04b-Methodology-bk.tex <==
\vspace{-2mm}
\section{Experimental Methodology
}
\label{sec:methodology}

\vspace{-1mm}

%In this section, we describe the cycle accurate simulation framework, 

\subsection{Cycle Accurate Simulation Framework}



In order to evaluate the dataflows, we built a cycle accurate simulation framework called OMEGA (\underline{\textbf{O}}bserving \underline{\textbf{M}}apping \underline{\textbf{E}}fficiency over \underline{\textbf{G}}NN \underline{\textbf{A}}ccelerators). Fig~\ref{fig:omega2} depicts the toolflow of the OMEGA framework.\footnote{We plan to open-source our framework after the paper is accepted. Its integration to PyTorch is also underway.}. OMEGA takes sparse graph of the workloads using CSR format and dimensions V, F and G as inputs.
OMEGA framework calls cycle accurate simulators for modelling GEMM and SpMM individually. The underlying hardware model of the cycle accurate simulator is similar to the flexible spatial accelerators MAERI~\cite{kwon2018maeri} and SIGMA~\cite{sigma}.
It consists of reconfigurable networks-on-chip 
for operand distribution % with distribution latency of one cycle  and the reduction is tree-based.
and output reduction allowing us to study different tile sizes. 
The cycle accurate simulator can support re-configurable spatial reduction and distribution sizes - thereby allowing us to study different tile sizes. 
The accelerator also has support for CSR decoding and indexing logic to run SpMM in addition to GEMM.
The simulator provides runtime, energy and activity counts for running SpMM and GEMM.
To model inter-phase dataflows, we built an analytical model around the cycle accurate simulator that computes the runtime, energy and buffering statistics of a GNN layer from the timestamps and intra-phase statistics from the simulator.
We modeled an accelerator with 512 PEs. The on-chip buffer size is 16 MB which is in the same ballpark as GNN accelerators~\cite{yan2020hygcn,liang2020engn}.

%The simulator can be used in both SpMM configuration and GEMM configuration and is used to compute the complete phases Aggregation and combination respectively. To implement inter-phase dataflows, we built an analytical model around the cycle accurate simulator that computes the runtime, energy and buffering statistics of a GNN layer from the timestamps and Intra-phase statistics from the simulator.%\SA{There is a conceptual break here.}

%\insertFigure{omega2}{OMEGA Tool Flow. %\EQ{@raveesh, reminder to update figure, controller to accelerator, inputs, etc.}}


%\PA{I would remove the previous para if we run out of space. Those are implementation details that can be omited }
%\SA{This seems incomplete or out of place?} 
%\TK{add some lines about underlying HW model}\Rav{@ Professor Krishna, I  have added a para am still thinking, whether we should add details about any specific underlying hardware here since we are exploring dataflows?}
%\TK{@Raveesh - i mean we should at least say we model a SIGMA-like accelerator that can be run either as Sparse for Aggre or Dense for Comb -- we are showing runtime in cycles so need to at least say how we estimated those}\Rav{Should we mention SIGMA here  YES :) ?}

%For Aggregation, the SpMM controller uses Compressed Sparse Row (CSR) format to store the adjacency matrix and it reduces only non-zero elements. It can support temporal reduction and it is also possible to configure the tile size for spatial reduction.

%In this work, since our goal is to compare the impact of the dataflows, we assume that there is sufficient buffering to run any dataflow to ensure that there are no stalls due to data fetches from the memory. Any performance difference is purely due to under-utilization of a dataflow, loading and streaming delays, and stalls in parallel pipeline dataflow.

%\SA{I find the flow hard to follow. Maybe this goes better at the beginning of the section? Like: we want to do this, and we do it with OMEGA.}
%\Rav{Actually, I was just trying to justify why we did on-chip}
%\SA{Right right. Just do what you think it's best. :)}\Rav{Actually the last sentence makes sense in 4C, I ll move it there}\Rav{\TODO{A line about on-chip data movement}}
%In this work, our purpose is to analyze the mapping characteristics of GNN workloads on the spatial accelerator compute engines. We characterize the on-chip data movement and runtime of GNN dataflows.
%\SA{The last sentence could maybe go to IV-C.}

%\subsection{Dataflow Evaluator}
\vspace{-1mm}

%\subsection{Candidate Dataflows}
%\vspace{-1mm}
%For evaluation, in the interest of space, 
we do a deep dive for 9 representative dataflows, listed in Table~\ref{tables:eval_config} using our taxonomy (Sec.~\ref{sec:dataflow}). All the configurations have phase order from Aggregation to Combination and vertex is always the outermost loop. For PP dataflow, we assume 
row-wise granularity %\TK{why do we only choose row gran?}\Rav{Loop order in STONNE} 
and since the number of vertices is high, it is possible to have different number of rows to have different impact. SP has vertex as the outer loop and feature as the inner loop because of the huge amount of memory saving in that order.
%The dataflow configurations have been named based on the taxonomy in Section~\ref{sec:taxonomy}.
Since we select a subset of choices, we also provide a compact  \textit{Name$^\dag$}
%\footnote{The compact name consists of three parts separated by '-'. First part represents inter-phase dataflow, second indicates dimensions which are necessarily spatial or temporal for Aggregation and the third part (if any) indicates dimensions which are necessarily spatial or temporal for combination. In third part of compact name for PP, the subscripts corresponding to the vertex are t/sl for lower(l) granularity and sh for higher(h) granularity. We also introduce High-V{\textsubscript{s}}-SP dataflow to highlight the problem of parallelizing sparse dimensions for all datasets except proteins and Mutag where T\textunderscore V is already high due to smaller T\textunderscore F limited by F.}
in Table~\ref{tables:eval_config} for the evaluation discussion.
%
% The compact name consists of three parts separated by '-'. First part represents inter-phase dataflow, second indicates dimensions which are necessarily spatial or temporal for Aggregation and the third part (if any) indicates dimensions which are necessarily spatial or temporal for combination. In third part of compact name for PP, the subscripts corresponding to the vertex are t/sl for lower(l) granularity and sh for higher(h) granularity.
% We also introduce High-V{\textsubscript{s}}-SP dataflow to highlight the problem of parallelizing sparse dimensions for all datasets except proteins and Mutag where T\textunderscore V is already high due to smaller T\textunderscore F limited by F. %Table~\ref{tables:eval_config}\footnote{Our purpose here is to not compare HyGCN and EnGN's underlying implementation. We evaluate HyGCN-like (PP) and EnGN like (SP) dataflows to understand the factors affecting the runtime associated with the dataflows.} describes all the configurations that we use for evaluations.

\input{tables/new/eval_config}

\input{tables/new/workload}

%\subsection{Target Datasets}


%Table~\ref{tables:workload} describes the datasets~\cite{kersting2016benchmark,yanardag2015deep} we use.
%in our evaluations.
%For graph classification, we use a batch size of 64 graphs for Protein, Mutag, Imdb-BIN and Collab and batch size of 32 for Reddit-bin \cite{kersting2016benchmark}. For node classification, we use Cora and Citeseer \cite{yanardag2015deep}.

%\TK{@Raveesh - Add a note about two assumptions: since the goal is to contrast dataflows, we assume (i) accelerator can run any of the dataflows, and (ii) there is enough buffering such that not there are no stalls due to data fetches from main memory. Any performance difference is purely due to under-utilization or stalls due pipeline dependence}\Rav{I have added it to Section 4A, comment there too to indicate the location}

\subsection{GNN Algorithms and Datasets}
We evaluate the dataflows described in Table~\ref{tables:eval_config} for GCN\cite{kipf2017semisupervised} for the
target datasets described in Table~\ref{tables:workload}. These are standard datasets representing workloads from multiple domains like biochemistry, citation networks and social networks \cite{kersting2016benchmark, yanardag2015deep}.
%\TK{add a line about these datasets being standard etc and representing multiple domains and cite where you got them from.}\Rav{@Eric, can you please cite, where you got the datasets from ?}
We evaluate one batch of 64 graphs for graph classification workloads (batch of 32 graphs for RedditBIN) and we evaluate node classification datasets Citeseer and Cora. 
%\TK{@Raveesh - you could add a line about graph data sets already sliced to fit on-chip buffers and cite that other paper that uses this line}\Rav{Generally accelerator papers propose slicing mechanisms}
The large graph sets are generally sliced to fit on-chip~\cite{yan2020hygcn,liang2020engn}. Large graph classification datasets can be batched such that the graphs fit on-chip.
For this work, there is sufficient on-chip buffering for a batch of graph classification datasets and for node classification datasets. We characterize on-chip data movement and runtime of the GNN dataflows since our aim is to study the behaviour of these dataflows on spatial accelerator.
%\TK{i meant just add citations here. There was a paper you showed that said graphs are sliced to fit on-chip memory etc. Just cite that paper after this point, and also cite HyGCN etc}
%Based on the dimensions and the observed results in the Section~\ref{sec:evaluation}, these workloads fall into three categories as shown in Table~\ref{tables:workload_cat}. %GS%We also evaluate the dataflows for GraphSage\cite{hamilton2017inductive} on datasets Collab and Cora. In GraphSage(GS), the neighbors are sampled to a fixed number, so the computation for Aggregation is more regular compared to GCN.Combination phase has two components, combination on the Aggregated matrix and combination on the input matrix.
For each dataflow, we also selected appropriate tile sizes as described below to create a complete mapping. 

==> 06-RelatedWork.tex <==
%\vspace{-1mm}
\section{Related Work}
\label{sec:relatedwork}
%\vspace{-1mm}
%\TK{make it crisper}\Rav{In addition to GNN Accelerators, we could discuss DNN dataflow exploration works}
%GNNs, given their utility in learning complex relationships from data-sets that can be represented as graphs, have attracted significant attention since 2018 to accelerate their computation \cite{abadal2020computing}. Correspondingly, in this section we highlight some of the most significant works with regards to GNN Accelerators as well as the mapping and scheduling of GNNs.         
%\TODO{@Sergi, Robert, Akshay} 
%\subsection{GNN Accelerators}
\Rav{Related work is not that big, this could be part of background ?}

\textit{\textbf{Dataflow Analysis.}} 
%\TK{Shorten this .. just point to Figure 2}
Prior dataflow works (such as Timeloop \cite{timeloop}, Interstellar \cite{interstellar}, and Kwon et al \cite{kwon2019understanding}) only analyze single-phase dense dataflows. As Fig.~\ref{fig:venn} shows, these dataflows are a subset of the GNN dataflows that we study.

\begin{comment}
\textit{\textbf{GNN Acceleration: Software Techniques.}}
%The acceleration of GNN workloads is an active area of research that distinguishes between software and hardware acceleration \cite{abadal2020computing}. On the one hand,
Software acceleration for GNNs aims at exploiting the knowledge of the graph properties to better adapt the workload to the underlying hardware \cite{Ma2019,gnnadvisor,Tripathy2020,greta,fey2019fast,wang2019deep,Zhu2018ali,Tian2020,hu2020featgraph,jia2019redundancy, chen2020rubik,abadal2020computing}. This includes techniques such as intelligent partitioning \cite{Tian2020}, sparsity-aware workload management \cite{gnnadvisor}, vertex reordering \cite{chen2020rubik}, or the caching of partial Aggregations to avoid redundant sums \cite{jia2019redundancy}. These techniques are either specific for GPUs, such as the dataflow constructs in Neugraph \cite{Ma2019}, or orthogonal to 
the approach of this paper. 
\end{comment}

\textit{\textbf{GNN Accelerators:}}
%\TK{the following para has too much detail. We just need a laundry list of GNN accelerators, no need for detaailed explanations for each since this is not an arch paper. Can we summarize to 2-3 lines?}
%On the other hand, hardware accelerators employ specific architectures to combat the alternating dense--sparse phases of GNNs and to adapt to their time-varying needs
%\cite{liang2020engn,yan2020hygcn,geng2019awb,Kiningham2020,Auten2020,Zeng2020,chen2020rubik, gcnax, iscas}. 
%These accelerators are developed by adhering to the characteristics of the GNN model, such as GCN, etc., to be processed as well as the underlying sparsity and size of the graph.
%The existing accelerators tackle the challenge in various ways. 
%EnGN \cite{liang2020engn}, HyGCN \cite{yan2020hygcn}, etc., provision vastly different methodologies to process GCN. 
%For instance, EnGN \cite{liang2020engn} relies on a unified architecture to perform both Aggregation and Combination efficiently, 
%a single compute engine alongside sparsity aware data caches, to minimize access to the main memory, 
%whereas HyGCN \cite{yan2020hygcn} utilizes two separate engines to that end. 
%for the Combination and Aggregation phases of the GCN computation. 
%Furthermore, in HyGCN, the properties of the systolic array as well as pipelining based optimization have been utilized to provision speed ups. Moreover, and as already stated above, methods such as GReTA \cite{greta} provision a software framework for executing GNNs on the underlying hardware engine through efficient partitioning and mapping of the graph.    
%Auten \emph{et al.} propose an architecture similar to HyGCN, but less integrated \cite{Auten2020}. Processing elements are grouped in tiles, allowing to scale-out the architecture if needed. AWB-GCN \cite{geng2019awb}, instead, provides multiple ways to alleviate the imbalance stemming from the skewed connectivity of widespread graphs .
%Centaur \cite{hwang2020centaur} tackles both dense and sparse computations, although not aiming directly at GNNs. Finally, we highlight GRIP \cite{Kiningham2020} as being among the first accelerators to explicitly consider edge updates. %\SA{@Tushar, @Raveesh, @Eric: please review this paragraph and modify it to better suit the motivatin of the paper} 
%Hardware techniques for accelerating GNNs include novel microarchitecture and dataflows. 
Each GNN accelerator implements a %\RB{"inherent"?} 
specific dataflow, which is generally fixed and not formally defined \cite{abadal2020computing,liang2020engn,yan2020hygcn,geng2019awb,Kiningham2020,Auten2020,chen2020rubik, gcnax, iscas}. Recently, GCNAX~\cite{gcnax} proposed a flexible accelerator with Design Space Exploration to choose the most energy efficient dataflow for a workload. 
%GCNAX supports variable loop orders and can turn on/off loop fusion and it treats both phases as SpMM.
GCNAX primarily targets off-chip dataflows with small Global buffers and 16 PEs, while our work primarily focuses on the on-chip dataflow strategies for large programmable spatial accelerators.
% This work, to the best of our knowledge, is the first to formalize a taxonomy and hardware evaluation methodology that can applied across a suite of existing and future GNN accelerators.  
%Recently, GCNAX~\cite{gcnax} proposed a flexible accelerator with Design Space Exploration to choose the most energy efficient dataflow for a workload. GCNAX supports variable loop orders and can turn on/off loop fusion and it treats both phases as SpMM. Recently, there has also been work on analytical modelling of data movement for GNN accelerators \cite{iscas}. %In addition, these works while presenting efficient architectures and frameworks, are very specific, and hence, a more generalized and global view of the different types of dataflows involved and possible for computing a GNN in an accelerator largely remains missing from literature.  



%\TK{Pls add papers like Timeloop, Interstellar, MAESTRO that perform dataflow analysis for spatial accelerators .. but say they focus on single independent kernels (like GEMM), not multi-phase like this work. And add that none of them targets sparsity}


%The acceleration of GNN workloads is an active area of research that distinguishes between software and hardware acceleration \cite{abadal2020computing}. In general, software acceleration for GNNs aims at exploiting the knowledge of the graph properties such as \textit{Sparsity} and their size so as to adapt and scale their computation on the underlying hardware engine as effectively as possible \cite{Ma2019,gnnadvisor,Tripathy2020,greta,fey2019fast,wang2019deep,Zhu2018ali,Tian2020,hu2020featgraph}. On the other hand, hardware accelerators provision a speed up in GNN computing through their specific architectural designs \cite{liang2020engn,yan2020hygcn,geng2019awb,Kiningham2020,Auten2020,Zeng2020}. These accelerators are developed by adhering to the characteristics of the GNN model, such as GCN, etc., to be processed as well as the underlying sparsity and size of the graph.

%However, to the best of our knowledge, none of the listed works formalize the taxonomy for the dataflows for GNN accelerators. In addition, these works while presenting efficient architectures and frameworks, are very specific, and hence, a more generalized and global view of the different types of dataflows involved and possible for computing a GNN in an accelerator largely remains missing from literature.  

%\textcolor{red}{AJ: TODO--> Add the papers here from the survey paper as refs., and extend discussion on some important works and how we are different.}

%\subsection{GNN Mapping and Scheduling}
%While specific works related to GNN dataflows do not currently exist in literature, multiple works, such as \cite{Zhu2018ali,jia2020improving,gnnadvisor,Tian2020, liang2020engn, geng2019awb}, propose methods to speed up graph processing through efficient mapping and scheduling strategies.  

%GNNs require efficient partitioning methods to cut down large graphs so that they fit within the caches and, therefore, process the graph efficiently. In this context, partition mapping and scheduling are essential to avoid slowing down the GNN processing and several works have investigated multiple alternatives \cite{Zhu2018ali,jia2020improving,gnnadvisor,Tian2020, liang2020engn, geng2019awb}. For example, in \cite{Zhu2018ali}, four different graph partitioning strategies are compared. In addition, EnGN and HyGCN introduce a graph partitioning and scheduling strategy to load and process large graphs. Specifically, in EnGN the graph is partitioned into a fixed number of tiles, and then considering how the data has to be reused, scheduling of either column or row of tiles is done first. A methodology to specify the benefits of either process has also been provisioned in \cite{liang2020engn}. Next, in HyGCN, a more dynamic method for graph partitioning has been provisioned wherein the objective is to eliminate sparsity from within tiles. Other methods such as \cite{geng2019awb} and \cite{Tian2020}, utilize the power law graph principles and the sparsity of the matrices to perform scheduling and mapping of the graph processing tasks.             % \TODO{CHECK if this is OK}


%For example, in \cite{Zhu2018ali}, four different graph partitioning strategies have been adopted so as to optimize the processing, as well as caching of highly connected vertices in multiple machines has been performed. This as a result reduces the requirement to access the main memory and avoid delays due to misses as well as access. In addition, EnGN and HyGCN introduce a graph partitioning and scheduling strategy to load and process large graphs. Specifically, in EnGN the graph is partitioned into a fixed number of tiles, and then considering how the data has to be reused, scheduling of either column or row of tiles is done first. A methodology to specify the benefits of either process has also been provisioned in \cite{liang2020engn}. Next, in HyGCN, a more dynamic method for graph partitioning has been provisioned wherein the objective is to eliminate sparsity from within tiles. Other methods such as \cite{geng2019awb} and \cite{Tian2020}, utilize the power law graph principles and the sparsity of the matrices to perform scheduling and mapping of the graph processing tasks.             
%\TODO{CHECK if this is OK}

%\SA{If we need to include more meat, we could talk about DNN dataflows and accelerators? But perhaps you guys are more knowledgeable on that?}

==> bk-05a-ArchVision.tex <==
\section{Architecture Implications}
\label{sec:archdesign}
%\Rav{SP works well but SP itself is large and flexibilty within SP is needed by means of flexible NoC}
%\Rav{Cora/Citeseer PP runtime}

To enable different dataflows, we propose a flexible accelerator with the following characteristics: 

\squishlist
\item {A flexible Network-On-Chip (NoC) for Intra-phase dataflows which adds the ability to support reduction and distribution of variable tile sizes for each dimension like in MAERI{~\cite{kwon2018maeri}} and SIGMA{~\cite{sigma}}. This will always be helpful whatever the inter-phase dataflow since intra-phase metrics depend on tile sizes.}
\item {Supporting variable sized splitting of a substrate into two phases for parallel pipelining which requires a flexible NoC and  homogeneous substrate. This is similar to what the AWB-GCN architecture proposes \cite{geng2019awb}.}
\item {The ability to support different inter-phase dataflows, a high-level architecture of which is shown in Fig.{~\ref{fig:substrate}}}
\item {The ability to turn off intermediate buffers when not needed for EnGN like SP dataflow to save energy.}
\item Using banked intermediate global buffers for low individual data access latency.
\squishend

\insertFigure{substrate}{Supporting multiple inter-phase dataflows in an accelerator.}

%\Rav{A section on "Architectural Vision" ? The "Insights from Evaluation" subsection would motivate flexible accelerator and Eric's figure} 


==> bk-05b-Eval-pact.tex <==
In this section, we discuss the impact of various dataflow choices like tile sizes and inter-phase dataflow on the runtime and energy. We analyze the runtime and energy for dataflow choices in Table~\ref{tables:eval_config} for workloads in Table~\ref{tables:workload}. We also find the best trade-off between performance and energy using the representative dataflows with multiple tile sizes. We also analyze the runtime of PP dataflows with variable allocation to understand the optimal load balancing between the two phases.


\insertWideFigure{Performance}{{Runtimes of Dataflows normalized to Seq-Nt for GCN algorithm. PE Utilization is close to 100\%. The values in the brackets are tile sizes for each dimension, represented as (T\textunderscore V{\textsubscript{AGG}},T\textunderscore N,T\textunderscore F{\textsubscript{AGG}},T\textunderscore V{\textsubscript{CMB}},T\textunderscore G,T\textunderscore F{\textsubscript{CMB}}).}}

\insertWideFigure{energy-int}{{On-Chip buffer access energies of dataflows, GB is Global Buffer and RF is local (PE) register file. Size of the Intermediate buffer for PP depends on the pipelining granularity. The values in the brackets are tile sizes for each dimension, represented as (T\textunderscore V{\textsubscript{AGG}},T\textunderscore N,T\textunderscore F{\textsubscript{AGG}},T\textunderscore V{\textsubscript{CMB}},T\textunderscore G,T\textunderscore F{\textsubscript{CMB}}}).}

\insertWideFigure{gb1}{{Global Buffer breakdown for Mutag and Citeseer, Adj-Adjacency matrix, Inp-Input matrix, Int-Intermediate matrix, Wt-weight matrix and Op-output matrix, Psum-partial sum accesses. The values in the brackets are tile sizes for each dimension, represented as (T\textunderscore V{\textsubscript{AGG}},T\textunderscore N,T\textunderscore F{\textsubscript{AGG}},T\textunderscore V{\textsubscript{CMB}},T\textunderscore G,T\textunderscore F{\textsubscript{CMB}}).}}%\TK{minor todo - pls rename RF to RF in this figure and wherever it appears in text. In text make it Register File (RF)}} \vspace{-2mm}}

\insertWideFigure{dse}{Runtime vs Energy plots for GNN dataflows. Granularity for PP = T\textunderscore V\textsubscript{MAX}.}

\insertWideFigure{ppvar}{Runtimes with different PE allocation to phases. Label represents the dataflow and the PE allocation ratio PE\textsubscript{AGG}-PE\textsubscript{CMB}. Runtimes are normalized to 50-50 low granularity. The values in the brackets are tile sizes for each dimension: (T\textunderscore V{\textsubscript{AGG}},T\textunderscore N,T\textunderscore F{\textsubscript{AGG}},T\textunderscore V{\textsubscript{CMB}},T\textunderscore G,T\textunderscore F{\textsubscript{CMB}}).}


%\insertWideFigure{performance-plots}{Normalized runtimes of GCN workloads. Runtimes are normalized by runtime of Seq-N\textsubscript{t} of the workloads and by Seq-N\textsubscript{s} for citeseer. Vertical axis represents dataflow compact names and tile sizes in order (T\textunderscore V\textsubscript{AGG},T\textunderscore N,T\textunderscore F\textsubscript{AGG},T\textunderscore V\textsubscript{CMB},T\textunderscore G,T\textunderscore F\textsubscript{CMB})}


%GS%\insertFigure{performance-plots-gs}{Normalized runtimes of some GraphSage workloads. Runtimes are normalized by runtime of SN\textsubscript{t}. Vertical axis represents dataflow compact names and tile sizes in order (T\textunderscore V\textsubscript{AGG},T\textunderscore N,T\textunderscore F\textsubscript{AGG},T\textunderscore V\textsubscript{CMB1},T\textunderscore G\textsubscript{CMB1},T\textunderscore F\textsubscript{CMB1}). The combination tiles, here represent combination of the aggregated feature vectors. We assume that combination of input feature vectors happens in parallel to this with same dataflow and allocated resources.}

%\subsection{Runtime Evaluation on Real Graph Structures}

%\subsection{Evaluation using Real Graph Structures}
\subsection{Runtime}
%\subsubsection{\textbf{Deep-dive: Runtime}}
We evaluate the dataflow configurations of Table~\ref{tables:eval_config} for the datasets of Table~\ref{tables:workload}. {Fig.{~\ref{fig:Performance}}} shows the GCN runtimes normalized by the delay of Seq-N\textsubscript{t} dataflow. %GS%%Figure~\ref{fig:performance-plots-gs} shows the evaluations for Collab and Cora for GraphSage algorithm. 
Our observations are as follows:

%\EQ{observation a bit too wordy, please bold the key sentences for each , so readers can quicky see which is important}\Rav{Good point, done}

%\vspace{2mm}
\squishlist

\item For Collab, spatial reduction (N\textsubscript{s}) in general performs much better than temporal reduction (N\textsubscript{t}), because Collab is densely connected. For Imdb, the performance is similar, which means that the optimal T\textunderscore N is within 1--10. For other datasets, since they are sparse, optimal T\textunderscore N is low. % Also, aggregation delay dominates in CL.
%GS%GraphSage (GS) for CL also has no underutilization since the number of neighbors are sampled to the same value. GS also has better PP performance because of faster Aggregation due to reduced neighbors.


\item SP-V\textsubscript{s}N\textsubscript{t}-V\textsubscript{s} performs well in most of the cases since parallelization of the vertices leads to reduced loading overhead. However, as observed in most of the datasets, specially in Reddit-bin, Citeseer and Cora, extremely high T\textunderscore V can lead to delays since the performance is limited by the a dense row (with large number of non-zeros) as demonstrated in High-V{\textsubscript{s}}-SP dataflow. Such dense row is referred to as "evil row" in AWB-GCN~\cite{geng2019awb}.

\item For the PP dataflow, spatial or temporal reduction has more impact on runtime compared to the granularity of pipelining. This is because the pipelining delay is dominated by the slower phase and the non-overlapping extra delay is that of a faster phase.

\item For all datasets, SP-F\textsubscript{s}N\textsubscript{t}-F\textsubscript{s} and PP-N\textsubscript{t}-V\textsubscript{t/sl} have tilings such that PP-N\textsubscript{t}-V\textsubscript{t/sl} computes both phases in parallel with half the feature tile size compared to SP-F\textsubscript{s}N\textsubscript{t}-F\textsubscript{s}. Yet both SP-F\textsubscript{s}N\textsubscript{t}-F\textsubscript{s} and PP-N\textsubscript{t}-V\textsubscript{t/sl} display different characteristics across different workloads. 

\item For the datasets Reddit-Bin and Cora, PP with high granularity has the best runtime, while for datasets Collab, Proteins, Mutag, SP dataflow with spatially mapped vertices has the best performance. Thus, different inter-phase dataflows can have optimal performance for different workloads.

\item For the Collab dataset, PP performs worse than Seq dataflow. This is due to poor load balancing between Aggregation and Combination. Thus, the ratios in which PEs are allocated to each phase is also essential to PP.

\squishend
%\vspace{2mm}
%\SA{This orphan sentence is intended? If so, you could start by "For all this, we conclude that..."}
%For all this, we conclude that the impact of a mapping or a tile size is highly dependent on the graph structure.%GS% and the GNN Algorithm being used. 
%There is no single best mapping that works well for all workloads.
%\TODO{also add a chart for GraphSAGE}
%\Rav{Footnote saying that we are not comparing EnGN and HyGCN and we are only contrasting the dataflows that they follow. Specific details of communication, sparsity handling etc. are not considered ????}
%\Rav{Footnote saying that our aim is not to find the best mapping(s) for a workload, but to understand the impact of tile sizes and dataflows}

%\subsubsection{\textbf{Deep-dive: Data Movement and Energy}}
\vspace{-2mm}
\subsection{Data Movement and Energy}
\vspace{-1mm}
%\insertWideFigure{energy}{{On-Chip Buffer access energies of Dataflows, GB is Global Buffer and RF is local (PE) buffer}}


%This subsection discusses the on-chip data movement across GNN dataflows, which translates to energy.
Fig{~\ref{fig:energy-int}} shows the energy consumed by various dataflows across workloads.
The energy difference comes due to 
differences in number of accesses 
across the memory hierarchy.
We assume the energy of a global buffer (GB) access to be 1.046pJ and the energy of a local PE register file (RF) access to be 0.053pJ based on the energy model from Dally \emph{et al.}{~\cite{ProfDallyTalk}}. For PP dataflow, we assume that there is a separate ping-pong buffer for intermediate data and the size of that depends on the capacity required based on Table~\ref{tables:inter_equations}. Some of the observations related to energy are as follows:
\squishlist
\item {Energy is dominated by GB reads followed by RF reads.}
%\item {Energy trends for T\textunderscore N are similar to performance across applications. Collab favors high T\textunderscore N while most of the others favor low T\textunderscore N.}

\item SP and PP have lower energy compared to Seq dataflow since these dataflows do not incur high intermediate global buffer accesses.

\item Fig~\ref{fig:gb1} shows the GB access breakdown for the workload. Datasets like proteins and mutag have a good proportion of Intermediate accesses which can be optimized by SP/PP, while on the other extreme, collab has extremely low intermediate accesses in Seq. This is because collab is relatively dense and most of the accesses are the input feature map accesses. Citeseer and Cora are small graphs with high number of features, so they have a lot of accesses in the combination phase which reduces the proportion of intermediate accesses in Seq.

\item Having high T\textunderscore V reduces the memory accesses in the combination phase. Although as T\textunderscore V increases, partial sum accesses increase due to low T\textunderscore F.

%\item  Comparing Seq-N\textsubscript{t} and PP-N\textsubscript{t}-V\textsubscript{t/sl}, in both the cases only, the Inter-phase dataflow is different, both parallelize features. Yet in Fig~\ref{fig:energy-int}, there is a noticeable difference between the energies and that is due to the size of the global buffer needed for Intermediate data. The difference is more significant in proteins and mutag where the adjacency matrices are sparse and number of features are low. 

\item High T\textunderscore V\textsubscript{CMB}, i.e., high granularity, reduces the Weight accesses considerably due to spatial reuse of vertices in DenseGEMM. In datasets like Citeseer and Cora, this effect significantly outweighs the energy due to large intermediate buffer. This shows that both tile sizes and inter-phase dataflows can be critical.

\item In PP dataflow, even though the accesses are same as Seq dataflow, we observe lower intermediate data energy since the intermediate data uses a smaller buffer and the energy of the memory accesses from smaller buffer is less.
\squishend
%\TODO{need a graph showing interm. 
%buffer accesses for all dataflows for various workloads}


%The following subsection discusses the amount of intermediate buffers required for various dataflows. This can serve as a proxy for additional energy overhead of inter-phase dataflows as the size of intermediate storage can determine the way, intermediate data is stored in memory hierarchy as shown in Fig~\ref{fig:MemHrch}. Table~\ref{tables:inter_equations} describes the analytical equations for intermediate buffering requirement for inter-phase dataflows.

%Sequential dataflow always has intermediate buffering requirement of V$\times$F since it needs to store the whole output. For large graphs and feature sizes, data cannot be buffered on-chip and is stored across memory hierarchy leading to high evergy overhead. Sequential pipeline dataflow SP\textsubscript{AC}(V\textsubscript{x}F\textsubscript{x}N\textsubscript{t},V\textsubscript{x}F\textsubscript{x}G\textsubscript{t}) has no intermediate buffering overhead since intermediate data generated locally in PEs is used by next phase, so no additional energy overhead. In Parallel Pipeline dataflow buffering depends on \textit{PPel}. For example, in row wise granularity, increase in T\textunderscore V\textsubscript{max} increases buffering overhead and hence energy.

%\subsection{Pipeline reusability}
%\SA{I'm not sure whether this section is needed. I mean, the pipeline reusability metric is not plotted or calculated anywhere, is it? If we propose a metric that helps evaluate or predict something, it should be calculated. Otherwise, we are just using space. This could be a  appendix?}
%For Seq dataflow, depending on the tile sizes and the workload, the amount of reuse that one gets from doing pipelining (Pipeline reusability - $\mathcal{P}$) can be defined as follows:

%\begin{equation}
 %  \mathcal{P} = \tfrac{mI_{WR}+mI_{RD}}{mA_{RD}+mX_{RD}+mI_{WR}+mI_{RD}+mW_{RD}+mX1_{WR}}.
%\end{equation}



%Here m(Matrix)\textsubscript{RD/WR} represents read/write buffer accesses of matrices; A(adjacency matrix), X(Input feature matrix), I(Intermediate matrix), W(Weight matrix) or X1(Output feature matrix). $\mathcal{P}$ represents the proportion of global memory accesses that can be done at a lower energy using a smaller buffer (PP or SP-arbitrary) or inside local PE register files (SP-EnGN-like).

%Pipeline reusability explains the relative energy saving that we get by pipelining using various intra-phase dataflows and on various workloads as shown in Fig~\ref{fig:energy-int} and Fig~\ref{fig:gb1}. Collab dataset has a lower pipeline reusability because the input feature accesses dominate. Since there is no spatial reuse in input feature accesses due to irregularity, input feature accesses, for most workloads are the major source of buffer accesses in our evaluations. Datasets like Citeseer and Cora are sparse, though, due to high F, they can spend significant amount of energy in weight reads depending on the intra-phase dataflow. Mutag and Proteins offer significant reuse opportunity, thus the amount of energy reduction that we get due to pipelining is significant.

%\vspace{-2mm}
\subsection{Design-space Exploration}
%\subsubsection{\textbf{Design-space of Runtime and Energy}}
\vspace{-1mm}
We have explored the performance and energy metrics of the GNN workloads individually. Fig.~\ref{fig:dse} shows performance vs energy plot to find the dataflows with right performance and energy trade-off. We profile multiple tile sizes for dataflow strategies in Table~\ref{tables:eval_config}. Our observations are as follows-
\squishlist
\item For Collab, SP-V\textsubscript{s}N\textsubscript{t}-V\textsubscript{s} is the optimal point for both performance and energy, although there is an optimal T\textunderscore V beyond which runtime increases due to effects of evil row and energy increases due to partial sum buffer accesses. 

\item For Collab, Seq-N\textsubscript{s} has low runtime but incurs high energy. PP dataflow in general has high runtime for collab dataset.

\item For Mutag, T\textunderscore F is limited by the number of features (F) which is 28. So most of the points have high T\textunderscore V. SP-V\textsubscript{s}N\textsubscript{t}-V\textsubscript{s} is the best trade-off between performance and energy but here, the performance does not reduce due to high T\textunderscore V unlike Collab since Mutag does not have very dense rows. Therefore the trend for optimal T\textunderscore V is also different from Collab.

\item For Mutag, Seq dataflow has high energy. PP dataflow has low energy and it is close to the energy of SP dataflow.

\item For Citeseer, most PP dataflow and SP-F\textsubscript{s}N\textsubscript{t}-F\textsubscript{s} have the best performance-energy tradeoff.

\item Energy and runtime of SP-V\textsubscript{s}N\textsubscript{t}-V\textsubscript{s} increases considerably as T\textunderscore V increases. 

\squishend

%\subsubsection{\textbf{Sensitivity Study: Load balancing in PP dataflow}}
\subsection{Sensitivity Study: Load balancing in PP dataflow}

%\SR{Did we define PE partitioning before ?}\Rav{I just meant variable allocation}
In PP dataflow, the delay is decided by the slower phase. Therefore load balancing is critical. Fig~\ref{fig:ppvar} shows the performance of different allocations PEs to phases for different pipeline granularities. Collab has higher density hence, slow Aggregation therefore 25-75 performs poorly. Mutag is sparse and also has low number of features and 50-50 is best allocation scheme amongst the three. Since, citeseer is sparse and has high number of features, combination phase is slower, therefore 75-25 allocation performs poorly.


\begin{comment}
\subsection{Summary of key findings}

Based on our observations and the dimensions, the workloads we evaluate fall into three categories as shown in Table~\ref{tables:workload_cat}. For the profiled loop orders in Table~\ref{tables:eval_config} and phase order Aggregation to Combination, we briefly summarize the performance and energy characteristics across three categories. %\EQ{are the categories mutually exclusive, couldnt a graph fit in both category 1 and category 2? also would be nice to define what is 'dense' and what is 'extremely sparse', maybe have an approximate density range.} 

\input{tables/new/workload_cat}


\textit{\textbf{Performance}}: For workloads with high number of features (Category 2), we observe that PP dataflow with high granularity of pipelining performs the best. For other two categories of workloads (Categories 1 and 3) which don't have high number of features, SP-V\textsubscript{s}N\textsubscript{t}-V\textsubscript{s} performs the best, although there is an optimal T\textunderscore V for best performance. Load balancing Agg and Cmb is critical for runtime of PP dataflow.

\textit{\textbf{Energy}}: For workloads in Category 1, SP-V\textsubscript{s}N\textsubscript{t}-V\textsubscript{s} has the lowest energy, although energy saving achieved by pipelining is not very significant. For workloads in Category 2, SP-V\textsubscript{s}N\textsubscript{t}-V\textsubscript{s} and PP-N\textsubscript{t}-V\textsubscript{sh} have the best energies and these dataflows have extremely close energies. However, High-V\textsubscript{s}-SP incurs high energy which means there is an optimal T\textunderscore V for which energy is the lowest. For workloads in Category 3, SP-F\textsubscript{s}N\textsubscript{t}-F\textsubscript{s} has the lowest energy and the energy of PP-N\textsubscript{t}-V\textsubscript{t/sl} dataflow is extremely close.

\textit{\textbf{Data movement}}: Dataflows of workloads in Category 1 spend a lot of accesses reading the input matrices since these workloads are relatively dense. Some dataflows of workloads in Category 2 spend a lot of accesses in weight reads, since they have large number of input features. Workloads in categories 1 and 2, incur little intermediate accesses, hence little reuse benefit of pipelining. Workloads in Category 3 do not incur significant proportion of accesses for input or weight matrix and allow more data to be reused by pipelining.

\textit{\textbf{Design Space Exploration}}: For workloads in category 1, the optimal point with respect to performance and energy is SP-V\textsubscript{s}N\textsubscript{t}-V\textsubscript{s}, however, with an optimal T\textunderscore V. Higher T\textunderscore V increases the runtime (evil row) and energy (partial sum accesses). For Category 2, PP dataflow in general and SP-F\textsubscript{s}N\textsubscript{t}-F\textsubscript{s} find the right performance-energy trade-off.  For category 3, the optimal point is SP-V\textsubscript{s}N\textsubscript{t}-V\textsubscript{s}, but unlike category 1, high T\textunderscore V increases only energy but it still reduces the runtime.
\end{comment}
%\subsection{Takeaways from the evaluation}

%Graph datasets have highly irregular structures which even amongst datasets are different. {We have observed in the evaluations using both synthetic and real workloads that tile sizes are critical to performance and energy. In terms of energy, SP-V{\textsubscript{s}}N{\textsubscript{t}}-V{\textsubscript{s}} works well, however there is an optimal T\textunderscore V for which the energy is the best. Energies of PP dataflows are close to the energies of SP dataflows. In terms of runtime, SP works well for low F (but there is an optimal T\textunderscore V) but PP works well for high F  (RedditBIN, Cora, Citeseer) with high T\textunderscore V{\textsubscript{CMB}}. For runtime and energy, there is an optimal T\textunderscore V in SP dataflow. Parallelizing V dimension improves latency, however the performance can be limited by evil row if T\textunderscore V is too large. From energy perspective, high T\textunderscore V reduces the weight reads but also increases the partial sum accesses (due to low T\textunderscore F) as shown in Fig{~\ref{fig:gb1}}.}

%{The choice of desired metric influences the design choices.} %GS% or every GNN algorithm.
%A denser graph will prefer spatial reduction while a sparser graph will prefer temporal. %Therefore, it would be beneficial to support flexible reduction capability like in MAERI\cite{kwon2018maeri} and SIGMA\cite{sigma}.
%Parallelizing V dimension improves latency, however the performance can be limited by evil row if the T\textunderscore V is too large. Therefore, either T\textunderscore V should be chosen carefully or an additional hardware support is required like in AWB-GCN\cite{geng2019awb}.
%{To achieve optimal energy, SP dataflow with flexible distribution network for variable T\textunderscore V, T\textunderscore F is a good choice and the energy of PP dataflow is also close. For performance, the optimal inter-phase dataflow is workload dependent.} For acceleration of all GNN workloads, we need a flexible\footnote{Note-By "flexibility" we mean configurability of tile-sizes and partition sizes, not Turing-completeness like CPUs/GPUs.} accelerator substrate for GNNs with an ability to choose various intra-phase parameters like tile sizes and also with the ability to model inter-phase dataflows - sequential pipeline and parallel pipeline.




==> bk-Future.tex <==
\section{Extensions and Future work}
\label{sec:archvision}


\textbf{\textit{Accelerator Architecture Implications}} - %Graph datasets have highly irregular structures which even amongst datasets are different. We have observed in the evaluations using both synthetic and real workloads that tile sizes are critical to performance and energy. We also observed that the inter-phase dataflow strategy affects the performance and energy of GNN dataflows.
We observed the performance and energy implications of various for different categories of graph workloads. The choice of desired metric influences the design choices. %GS% or every GNN algorithm.
%A denser graph will prefer spatial reduction while a sparser graph will prefer temporal. %Therefore, it would be beneficial to support flexible reduction capability like in MAERI\cite{kwon2018maeri} and SIGMA\cite{sigma}.
%Parallelizing V dimension improves latency, however the performance can be limited by evil row if the T\textunderscore V is too large. Therefore, either T\textunderscore V should be chosen carefully or an additional hardware support is required like in AWB-GCN\cite{geng2019awb}.
The choice of dataflow is also dependent on the workload. This suggests that efficient acceleration of all GNN workloads requires flexible
%\footnote{Note-By "flexibility" we mean configurability of tile-sizes and PE-partition sizes, not Turing-complete programmability like CPUs/GPUs.}
accelerator substrate for GNNs with an ability to choose various intra-phase parameters like tile sizes and also with the ability to run inter-phase dataflows - SP and PP, rather than design for one dataflow like current GNN accelerators.
%Further, programmable accelerators like 
%SambaNova, Cerebras, GraphCore and so on are 
%promising platforms.
%MAERI~\cite{kwon2018maeri} supports configurability in tile sizes for intra-phase dataflows.
%\textbf{\textit{Exploration of hardware parameters}} - %In this work, we use OMEGA to explore the impact of different dataflow strategies for fixed hardware.
We can also leverage OMEGA to explore the design space of hardware parameters like buffer size, NoC bandwidth, number of PEs, NoC topologies for distribution/reduction etc for designing such accelerators.
%Scalability is another interesting area of research.

\textbf{\textit{Mapping Optimizer.}}
In this work, we analyzed select dataflows to demonstrate interesting insights.
%In this work we develop a taxonomy to characterize the design space of GNN dataflows and the OMEGA framework to model the GNN mappings.
A mapping optimizer can be built on top of the OMEGA framework which automatically searches the search space of the dataflows. There are existing mapping optimizers for DNN accelerators~\cite{interstellar, chatarasi2020marvel,kao2020gamma}. Since GNN dataflows add an additional inter-phase optimizations knob, dataflow exploration is important.



\textbf{\textit{Dataflows for Inter-phase sparse-dense models}} - Though this work focuses on GNNs,
%as an example because they demonstrate the importance of multiphase computations, dataflow selection and workload characterisitics. However,
the methods proposed can be generalized to dataflows for multiphase computations that are workload dependent (GEMM-GEMM/GEMM-SpMM/SpMM-SPMM). One immediate example is Deep Learning Recommendation Models\cite{naumov2019deep} that is built of a SpMM and DenseGEMM in parallel followed by concatenation followed by DenseGEMMs.

% In particular, since GNN consists of SpMM and a DenseGEMM, it is a wider generalization of a single GEMM or a single SpMM operation. The same ideas can also be extended to Facebook Deep Learning Recommendation Models\cite{naumov2019deep} which consists of SpMM and DenseGEMM in parallel followed by concatenation followed by DenseGEMMs. Moreover, the inter-phase analysis can also be extended to multiple GEMMs or multiple SpMMs.

%We choose GNNs as an example because they demonstrate the importance of all three critical aspects, their immediate impact to broad set of applications and a possibility to utilize dataflow choices of several special purpose accelerators. However, the methods proposed here could be generalized to other dataflows for multiphase computations that are workload dependent.


==> bk05-Synthetic.tex <==
\subsection{Analysis using Synthetic Matrices}

\insertWideFigure{synthetic}{(a) and (b) the impact of tile sizes on Aggregation (V\textsubscript{t}F\textsubscript{x}N\textsubscript{x}) runtime. Impact of tile size T\textunderscore N on performance for graphs with (a) V=10000 (High) and F=32 (low) and (b) F=512 (High) and V=1000 (Low) for varying average degrees (D). Number of PEs = 128. T\textunderscore V=1 and T\textunderscore F={128/T\textunderscore N}. Runtime is normalized by runtime correspoding to highest D and lowest T\textunderscore N. (c) and (d) show the Impact of factors affecting PP for Aggregation followed by Combination. V=1024, F=512 and G=16 and number of PEs=512 for each phase for different average degrees D. (c) shows the runtime for different tile sizes. Dataflow - PP\textsubscript{AC}(V\textsubscript{t}F\textsubscript{x}N\textsubscript{x}, V\textsubscript{t}G\textsubscript{s}F\textsubscript{s}). T\textunderscore N in the inter-phase pipeline. T\textunderscore V=1, T\textunderscore F\textsubscript{CMB}=32, T\textunderscore G=16, T\textunderscore F\textsubscript{AGG} = {512/T\textunderscore N}. (d) shows the variation of performance with the increase in granularity of pipelining. Dataflow- PP\textsubscript{AC}(V\textsubscript{t}F\textsubscript{s}N\textsubscript{t}, V\textsubscript{x}G\textsubscript{t}F\textsubscript{x}). V=1024,  T\textunderscore V\textsubscript{CMB} is varied and it represents the number of rows being pipelined. T\textunderscore F\textsubscript{CMB}=512/T\textunderscore V\textsubscript{CMB}. (e) shows the impact of factors affecting SP for Aggregation followed by Combination. Dataflow -  SP\textsubscript{AC}(V\textsubscript{x}F\textsubscript{x}N\textsubscript{t},V\textsubscript{x}F\textsubscript{x}G\textsubscript{t}). V=1024, F=512, G=16, Number of PEs = 512. These figures show the impact of different tile size combinations T\textunderscore V and T\textunderscore F. Sequential pipelining for T\textunderscore V = \{1,8,64,512\}. T\textunderscore V = 512/T\textunderscore V with T\textunderscore N = T\textunderscore G = 1. Note that this example does not aim to model exact EnGN implementation. Here, inter-phase dataflow is EnGN like.}

%\TODO{@Add a line saying we use synthetic workloads to underdstand tile sozes for some of the dataflows in Table II}\Rav{@Professor Krishna, first sentence}

In this subsection, we evaluate GCN\cite{kipf2017semisupervised} on synthetic matrices to understand the impact of tile sizes for some of the dataflows in Table~\ref{tables:eval_config}. The synthetic workloads used are based on GEMMs. Each of the synthetic adjacency matrices has a varying number of edges (i.e., GEMM sparsity ratio).

\subsubsection {Intra-phase dataflows} Here, we evaluate the factors that influence the performance of an individual phase. For the combination (Dense) phase, there is a vast literature describing Dense CNNs and Dense GEMMs and we refer the reader to Kwon \emph{et al.}\cite{kwon2019understanding} for more details.

%\insertFigure{gnn-agg}{Aggregation dataflow- V\textsubscript{t}F\textsubscript{x}N\textsubscript{x}. Impact of tile size T\textunderscore N on performance for graphs with (a) V=10000 (High) and F=32 (low) and (b) F=512 (High) and V=1000 (Low) for varying average degrees (D). Number of PEs = 128. T\textunderscore V=1 and T\textunderscore F={128/T\textunderscore N}. Runtime is normalized by runtime correspoding to highest D and lowest T\textunderscore N. \TK{Combinee Fig 9, 10 and 11 into a 2 column figure with shared legend.}}

For Aggregation (SpMM), two primary factors that influence the run-time are the set of tile sizes for various dimensions and the amount of sparsity. Large T\textunderscore N can lead to under-utilization of PEs. However, if T\textunderscore N=1, latency 
can be high specially when the second phase needs to use the output soon, for example, PP 
%\SA{Parallel Pipeline? This sometimes appears in full, sometimes as an acronym. It's confusing.}.
The impact of tile sizes on performance for different graphs is shown in Fig.~\ref{fig:synthetic}a-b. These plots show that as the graph becomes more densely connected, higher T\textunderscore N is more optimal. {Thus, the optimal tile size for reduction in SpMM depends on the graph sparsity.}

\subsubsection{Inter-phase dataflows}

%Here, we describe the factors affecting inter-phase dataflows. 
The factors affecting the performance of the Sequential dataflow are the same as the factors affecting dataflows of individual phases because the number of cycles is simply the sum of number of cycles of individual phases.

%The key factors that affect parallel pipeline are the factors governing the individual phases and the number of granularity at which the data is broken and pipelined. Factors governing individual phase affect the performance, as each pipeline iteration has runtime equal to that of the time taken by the slower phase. The number of elements that are spatially exchanged determines the buffer size required and the latency of the non-overlapping pipeline iteration. Here, we take row-wise granularity with loop order VFN, VGF with phase order Aggregation to Combination and evaluate the impact of spatial and temporal reduction and impact of number of rows computed before synchronization.

%\insertFigure{gnn-pp}{Impact of factors affecting PP for Aggregation followed by Combination. V=1024, F=512 and G=16 and number of PEs=512 for each phase for different average degrees D. (a) shows the runtime for different tile sizes. Dataflow - PP\textsubscript{AC}(V\textsubscript{t}F\textsubscript{x}N\textsubscript{x}, V\textsubscript{t}G\textsubscript{s}F\textsubscript{s}). T\textunderscore N in the inter-phase pipeline. T\textunderscore V=1, T\textunderscore F\textsubscript{CMB}=32, T\textunderscore G=16, T\textunderscore F\textsubscript{AGG} = {512/T\textunderscore N}. (b) shows the variation of performance with the increase in granularity of pipelining. Dataflow- PP\textsubscript{AC}(V\textsubscript{t}F\textsubscript{s}N\textsubscript{t}, V\textsubscript{x}G\textsubscript{t}F\textsubscript{x}). V=1024,  T\textunderscore V\textsubscript{CMB} is varied and it represents the number of rows being pipelined. T\textunderscore F\textsubscript{CMB}=512/T\textunderscore V\textsubscript{CMB}.}

In PP dataflow, the delay is governed by the slower phase. Therefore, intra-phase performance is critical to PP dataflow. PP dataflow is also affected by granularity as an increase in granularity leads to a growth of the delay of the non-overlapping part. Fig.~\ref{fig:synthetic}c shows the impact of temporal or spatial reduction in Aggregation on overall pipelining. For lower average degrees, the combination delay dominates the Aggregation and, thus, changes in T\textunderscore N do not impact the net delay. However, as the average degree increases, Aggregation delay starts to dominate and affect the net delay. %For low, medium and very low average degrees, combination delay dominates aggregation delay if the spatial tile size is low, so the spatial reduction does not have any impact, but as the spatial tile size increases, aggregation delay increases and starts dominating. For high average degree, aggregation delay dominates and the minimum delay is for a relatively large value of T\textunderscore N 
Fig.~\ref{fig:synthetic}d shows the impact of having high granularity on performance. On increasing T\textunderscore V\textsubscript{CMB}, the delay first decreases due to parallelization of the stationary dimension V, but increases because of the increase in the non-overlapping delay.

%\insertFigure{gnn-sp}{Impact of factors affecting SP for Aggregation followed by Combination. Dataflow -  SP\textsubscript{AC}(V\textsubscript{x}F\textsubscript{x}N\textsubscript{t},V\textsubscript{x}F\textsubscript{x}G\textsubscript{t}). V=1024, F=512, G=16, Number of PEs = 512. These figures show the impact of different tile size combinations T\textunderscore V and T\textunderscore F. Sequential pipelining for T\textunderscore V = \{1,8,64,512\}. T\textunderscore V = 512/T\textunderscore V with T\textunderscore N = T\textunderscore G = 1. Note that this example does not aim to model exact EnGN implementation. Here, inter-phase dataflow is EnGN like.}


For SP, we use EnGN-like dataflow. We evaluate this dataflow for phase order aggregation to combination for tile sizes T\textunderscore F and T\textunderscore V. Fig.~\ref{fig:synthetic}e shows the impact of different tile sizes T\textunderscore V and T\textunderscore F on interleaving. In this example, Aggregation and Combination %\SA{always capitalized?}
have vertices %\SA{a vertex? vertices?}
in the outermost loop. Thus, tiling T\textunderscore V spatially reduces the number of cycles needed to load vertices in the PEs, although the latency becomes higher beyond a certain point. The main reason is that V is an irregular dimension and parallelizing V implies that the computation is limited by the vertex with most neighbors in the tile, which is referred to as "evil row" in AWB-GCN{~\cite{geng2019awb}}. The impact of such "evil row" is more significant in real world graphs. AWB-GCN has a load balancing engine that schedules the evil row on multiple PEs. Alternatively, one can also choose lower T\textunderscore V.

{Thus we observe from the above analysis, that the choice of tile sizes has a huge impact on each dataflow and the optimal tile sizes can vary with the graph.}
%Since this is random sparsity, the impact of high T\textunderscore V is not severe here but real graph datasets have evil rows and higher T\textunderscore V implies that computation of the vertices parallelized is limited by the computation of evil row. More T\textunderscore V implies, more vertices being limited by evil rows. To deal with evil rows, AWB-GCN\cite{geng2019awb} has an workload balancing component that schedules evil row on multiple underutilized engines. However, choosing a relatively lower tile size can also dilute the impact of evil rows.


==> eval_config.tex <==
\begin{scriptsize}
\begin{table}[ht!]
  \centering
  \caption{Representative dataflow configurations for evaluation.}
  \label{tables:eval_config}
  \begin{tabular}{|l|l|l|}
    \hline
    \textbf{Dataflow Configuration} & \textbf{Name} & \textbf{Description}  \\
    \hline
    Seq\textsubscript{AC}(V\textsubscript{x}F\textsubscript{x}N\textsubscript{t},V\textsubscript{x}G\textsubscript{x}F\textsubscript{x}) & Seq-N\textsubscript{t} & Sequential dataflow \\ & & Temporal Aggregation \\
    \hline
    Seq\textsubscript{AC}(V\textsubscript{x}F\textsubscript{x}N\textsubscript{s},V\textsubscript{x}G\textsubscript{x}F\textsubscript{x}) & Seq-N\textsubscript{s} & Sequential dataflow \\ & & Spatial Aggregation\\
    \hline
    SP\textsubscript{AC}(V\textsubscript{x}F\textsubscript{s}N\textsubscript{t},V\textsubscript{x}F\textsubscript{s}G\textsubscript{x}) & SP-F\textsubscript{s}N\textsubscript{t}-F\textsubscript{s} & Sequential Pipeline dataflow \\ & & EnGN-like \\ & & Temporal Aggregation\\ & & Relatively high T\textunderscore F \\
    \hline
    %SP\textsubscript{AC}(V\textsubscript{x}F\textsubscript{s}N\textsubscript{s},V\textsubscript{x}F\textsubscript{s}G\textsubscript{x}) & SP-F\textsubscript{s}N\textsubscript{s}-F\textsubscript{s} & Sequential Pipeline dataflow \\ & & Spatial Aggregation\\ & & Relatively high T\textunderscore F \\
    %\hline
    SP\textsubscript{AC}(V\textsubscript{s}F\textsubscript{x}N\textsubscript{t},V\textsubscript{s}F\textsubscript{x}G\textsubscript{x}) & SP-V\textsubscript{s}N\textsubscript{t}-V\textsubscript{s} & Sequential Pipeline dataflow \\ & & EnGN-like \\ & & Temporal Aggregation\\ & & Relatively high T\textunderscore V \\
    \hline
    %SP\textsubscript{AC}(V\textsubscript{s}F\textsubscript{x}N\textsubscript{t},V\textsubscript{s}F\textsubscript{x}G\textsubscript{x}) & SP-V\textsubscript{s}N\textsubscript{s}-V\textsubscript{s} & Sequential Pipeline dataflow \\ & & Spatial Aggregation\\ & & Relatively high T\textunderscore V \\
    %\hline
    PP\textsubscript{AC}(V\textsubscript{x}F\textsubscript{x}N\textsubscript{t},V\textsubscript{x}G\textsubscript{x}F\textsubscript{x}) & PP-N\textsubscript{t}-V\textsubscript{t/sl} & Parallel Pipeline dataflow \\ & & Temporal Aggregation\\ & & HyGCN-like \\& & Granularity of lower rows \\
    \hline
    PP\textsubscript{AC}(V\textsubscript{x}F\textsubscript{x}N\textsubscript{s},V\textsubscript{x}G\textsubscript{x}F\textsubscript{x}) & PP-N\textsubscript{s}-V\textsubscript{t/sl} & Parallel Pipeline dataflow \\ & & Spatial Aggregation \\ & & Granularity of lower rows \\
    \hline
    PP\textsubscript{AC}(V\textsubscript{x}F\textsubscript{x}N\textsubscript{t},V\textsubscript{s}G\textsubscript{x}F\textsubscript{x}) & PP-N\textsubscript{t}-V\textsubscript{sh} & Parallel Pipeline dataflow \\ & & Temporal Aggregation\\ & & HyGCN-like \\ & &  Granularity of higher rows \\
    \hline
    PP\textsubscript{AC}(V\textsubscript{x}F\textsubscript{x}N\textsubscript{s},V\textsubscript{s}G\textsubscript{x}F\textsubscript{x}) & PP-N\textsubscript{s}-V\textsubscript{sh} & Parallel Pipeline dataflow \\ & & Spatial Aggregation\\ & & Granularity of higher rows \\
    \hline
    {SP{\textsubscript{AC}}(V{\textsubscript{s}}F{\textsubscript{x}}N{\textsubscript{t}},V{\textsubscript{s}}F{\textsubscript{x}}G{\textsubscript{x}})} & {High-V{\textsubscript{s}}-SP} & {SP dataflow with high T\textunderscore V} \\
    \hline
  \end{tabular}
\vspace{-3mm}
\end{table}
\end{scriptsize}

==> tables/dataflow_bk.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[]
\centering
\caption{Reuse opportunities for GEMM dimensions. (Intra-phase dataflow) \TK{the goal of this table is nice but I think we could simplify it and make it similar to Table II. @Eric - put a new table in "intra-phase dataflow" sheet in our spreadsheet. Can you put that here?}} %\TK{@Eric - can we replace this / augment this with a figure simply showing a GEMM mapped over a simple 2D array in a WS manner and show multicast of MK matrix, and spatial reduction across K?}}
\begin{tabular}{|l|l|l|l|l|l|l|l|l|l|l|l|l|l|}
\hline
\multicolumn{7}{|c|}{\textbf{Spatial}}                                                                                                                                                    & \multicolumn{7}{c|}{\textbf{Temporal}}                                                                              \\ \hline
\multirow{2}{*}{\textbf{Dimension}} & \multicolumn{3}{c|}{\textbf{Coupling}}                       & \multicolumn{3}{c|}{\textbf{Reuse}}                                                  & \multirow{2}{*}{\textbf{Dimension}} & \multicolumn{3}{c|}{\textbf{Coupling}} & \multicolumn{3}{c|}{\textbf{Reuse}}  \\ \cline{2-7} \cline{9-14} 
                                    & \textbf{B}         & \textbf{A}         & \textbf{O}         & \textbf{B}                 & \textbf{A}                 & \textbf{O}                 &                                     & \textbf{B}  & \textbf{A}  & \textbf{O} & \textbf{B} & \textbf{A} & \textbf{O} \\ \hline
\multirow{2}{*}{\textbf{M}}         & \multirow{2}{*}{}  & \multirow{2}{*}{Y} & \multirow{2}{*}{Y} & \multirow{2}{*}{Multicast} & \multirow{2}{*}{}          & \multirow{2}{*}{}          & K                                   & Y           & Y           &            &            &            & Reduction  \\ \cline{8-14} 
                                    &                    &                    &                    &                            &                            &                            & N                                   & Y           &             & Y          &            & Multicast  &            \\ \hline
\multirow{2}{*}{K}                  & \multirow{2}{*}{Y} & \multirow{2}{*}{Y} & \multirow{2}{*}{}  & \multirow{2}{*}{}          & \multirow{2}{*}{}          & \multirow{2}{*}{Reduction} & M                                   &             & Y           & Y          & Multicast  &            &            \\ \cline{8-14} 
                                    &                    &                    &                    &                            &                            &                            & N                                   & Y           &             & Y          &            & Multicast  &            \\ \hline
\multirow{2}{*}{N}                  & \multirow{2}{*}{Y} & \multirow{2}{*}{}  & \multirow{2}{*}{Y} & \multirow{2}{*}{}          & \multirow{2}{*}{Multicast} & \multirow{2}{*}{}          & M                                   &             & Y           & Y          & Multicast  &            &            \\ \cline{8-14} 
                                    &                    &                    &                    &                            &                            &                            & K                                   & Y           & Y           &            &            &            & Reduction  \\ \hline
\end{tabular}
\label{tables:dataflow}
\end{table*}

==> tables/inter_equations.tex <==
\begin{scriptsize}
\begin{table}[t]
  \centering
  \caption{Runtime and buffering requirements for inter-phase dataflows}%\Rav{There is space for remarks too if needed}}
  %\TK{@Raveesh - by x do you mean you can do either s or t for that dimension? So does that mean each row is actually multiple datapoints? Thats confusing.}\Rav{It means that the datapoint that we choose for evaluation of that dataflow can have varaible tile sizes for dimension marked by X. S and T on the other hand mean that its NECESSARILY spatial or temporal}}
  \label{tables:inter_equations}
  \begin{tabular}{|l|l|l|}
    \hline
    \textbf{Inter-phase} & \textbf{Intermediate} & \textbf{Runtime}  \\
    \textbf{dataflow} & \textbf{Buffering} & \\
    \hline
    %Seq & $V\times F$ & $t_{AGG}+t_{CMB}$\\
    %\hline
    Seq & V$\times$F & t\textsubscript{AGG}+t\textsubscript{CMB}\\
    \hline
    SP-arbitrary & $Computed\_V\times$ & t\textsubscript{AGG}+t\textsubscript{CMB}\\
    & $Computed\_F$ & \\
    \hline
    %SP-EnGN-like & $0$ & $t_{AGG}+t_{CMB}-t_{load}$\\
    %\hline
    SP-EnGN-like & 0 & t\textsubscript{AGG}+t\textsubscript{CMB}-t\textsubscript{load}\\
    \hline
    %PP-Element & $2\times T\_V\times T\_F$ & \\
    %\hline
    PP-elements & 2$\times$T\textunderscore V\textsubscript{max}$\times$T\textunderscore F\textsubscript{max} & sum(max(t\textsubscript{AGG},\\ & & t\textsubscript{CMB})\textsubscript{PPel})\\
    \hline
   PP-Row & 2$\times$T\textunderscore V\textsubscript{max}$\times$F & sum(max(t\textsubscript{AGG},\\ & & t\textsubscript{CMB})\textsubscript{PPel})\\
    \hline
    PP-Column & 2$\times$V$\times$T\textunderscore F\textsubscript{max} & sum(max(t\textsubscript{AGG},\\ & & t\textsubscript{CMB})\textsubscript{PPel})\\
    \hline
  \end{tabular}
\vspace{-3mm}
\end{table}
\end{scriptsize}

==> tables/interleave.tex <==
\begin{table*}[ht!]
\scriptsize
\centering
\caption{Characterizing the design-space of dataflows for GNN Accelerators (Note that any direction will affect the aggregation and combination dimension variables, but similar concepts apply). Subscript s, t, * means spatial, temporal, either spatial or temporal respectively. Curly brackets '\{\}' show that the loop order is interchangeable.} %\TK{what is intermediate support? maybe change to  ``Intermediate Buffer". For the NoC/PE support for PP, are we direvtly sending dataa from PEs doing aggr to PEs doing comb? thats what explanation sounds like. If yes, why do we need Interm Buffer? If not, then the NoC field should be about writing values to interm buffer after aggr and reading from it during comb}\Rav{Yes, changed to "support to connect agg and cmb units to intermediate buffers"}} %\Rav{Me - SP and Seq done and expanded PP, should we keep all 3 rows of table for cmb->agg or compact that piece ? } %\TK{@Eric / Raveesh -- for PP, isnt there any specific requirement from NoC or PE wrt multicast or spatial reduction, depending on the dataflow? Depends on accelerator seems vague} \Rav{Actually it depends on tiles, how about "Temporal reduction requires in-place accumulation support and spatial dimesnions require multicast/spatial reduce"}\TK{Yeah but thats just a general statement. Can you mention in each row which dimensions requires multicast distribution, and which requires spatial or temporal reduction? Similar to Fig 3b. Also -- for the SP row, ``in-place buffers" is vague. Do you mean ``Requires support for storing outputs of the aggregation stage locally in the PEs so they can be reused as inputs for the combination stage" ? if yes, can you say that}
%\TODO{Need to specify what {}, *, s and t subscripts mean} %\TODO{Shorten 3rd row NoC multicast and PE support}}

\begin{tabular}{lllllll}
\toprule
\textbf{Inter Phase}                                                                      & \textbf{Aggregation} & \textbf{Combination} & \textbf{\begin{tabular}[c]{@{}l@{}}Intermediate \\ Buffer\end{tabular}} & \textbf{NoC / PE Support}                                                                                                             & \textbf{\begin{tabular}[c]{@{}l@{}}Example \& \\ Order\end{tabular}}      & \textbf{Remarks}                                                                                                                                                                                                                                                                                           \\
\toprule
\textbf{\begin{tabular}[c]{@{}l@{}}Sequential\\ (Seq)\end{tabular}}            & \{V\textsubscript{*} F\textsubscript{*} N\textsubscript{*}\}         & \{V\textsubscript{*} G\textsubscript{*} F\textsubscript{*}\}         & \multicolumn{1}{c}\cmark      & Depends on accelerator                                                                                                               & \begin{tabular}[c]{@{}l@{}}TPU \cite{tpu-isca} \\ Eyeriss \cite{eyeriss2}\\ (any direction*)\end{tabular}     & \begin{tabular}[c]{@{}l@{}}Similar to running one full or tiled layer at a \\time. Outputs of one layer gets stored in \\scratchpad and rescheduled back into the PEs.\end{tabular}                                                                                                         \\ % \\
\hline
\textbf{\begin{tabular}[c]{@{}l@{}}Sequential\\ Pipeline \\ (SP)\end{tabular}} &  \{V\textsubscript{*} F\textsubscript{*}\} N\textsubscript{t}    & \{V\textsubscript{*} F\textsubscript{*}\} G\textsubscript{t}         & \multicolumn{1}{c}\xmark                                                                     & \begin{tabular}[c]{@{}l@{}}Requires support to\\ store phase 1 outputs \\locally inside PE, so \\ that phase 2 can use\\ them as inputs\end{tabular} & \begin{tabular}[c]{@{}l@{}}EnGN \cite{liang2020engn}\\ (any direction*)\end{tabular}          & \begin{tabular}[c]{@{}l@{}}No intermediate support required, as output data\\ of one phase is stationary in the buffers, and can \\ be used as input for the next phase. Order of V,F  \\ should be the same for both the phases. T\textunderscore V\textsubscript{AGG}=\\T\textunderscore V\textsubscript{CMB} and T\textunderscore F\textsubscript{AGG}=T\textunderscore F\textsubscript{CMB} and reduction\\ is temporal as data is always in in-place buffers. \end{tabular}                                                                                                   \\                      % \\
\hline
\textbf{}                                                                      & V\textsubscript{t} \{F\textsubscript{s} N\textsubscript{t}\}         & \{V\textsubscript{s} G\textsubscript{s} F\textsubscript{t}\}         &  \multicolumn{1}{c}\cmark        & \begin{tabular}[c]{@{}l@{}}Requires support to\\ store agg. phase outputs \\locally inside PE, so \\ that cmb. phase can use\\ them as inputs\end{tabular}                                                                                                        &     \begin{tabular}[c]{@{}l@{}}Rubik \cite{chen2020rubik} \\ (agg->cmb)\end{tabular}                                                                      & \begin{tabular}[c]{@{}l@{}} Paper also focuses on reducing redundant \\ aggregations by saving duplicate data onto a \\ private cache. Similar to EnGN, no intermediate \\ data reordering required  as output data of one \\ phase is stationary in PEs and is used as inputs \\ for the next phase. \end{tabular}                              

                                            \\      %                 \\
                                            \hline
\textbf{}                                                                      & \{V\textsubscript{*} F\textsubscript{*} N\textsubscript{*}\}         & \{V\textsubscript{*} G\textsubscript{*} F\textsubscript{*}\}         & \multicolumn{1}{c}\cmark       & 
\begin{tabular}[c]{@{}l@{}}Agg:V\textsubscript{s},F\textsubscript{s}  require multicast\\ distribution. N\textsubscript{s/t} requires\\ spatial/temporal reduction.\\ Cmb:V\textsubscript{s},G\textsubscript{s}  require multicast\\ distribution. F\textsubscript{s/t} requires \\ spatial/temporal reduction.  \end{tabular}  
&         (any direction*)                                                    & \begin{tabular}[c]{@{}l@{}}There will be a buffer/ setup delay between \\ aggregation and combination phases to remap\\ output data to new location.\end{tabular}     

\\                                                %    \\
\hline
\textbf{\begin{tabular}[c]{@{}l@{}}Parallel \\ Pipeline\\ (PP)\end{tabular}}   & \{V\textsubscript{*} F\textsubscript{*}\} N\textsubscript{*}         & \{V\textsubscript{*} F\textsubscript{*}\}  G\textsubscript{*}        & \multicolumn{1}{c}\cmark     & \begin{tabular}[c]{@{}l@{}}Need support to connect \\agg and cmb units to\\ intermediate buffer\end{tabular}                                                          & \begin{tabular}[c]{@{}l@{}}(agg -\textgreater cmb)\end{tabular} & \begin{tabular}[c]{@{}l@{}}\textbf{Element(s) wise granularity}: Element(s) of the \\ intermediate matrix indexed by V,F can be \\ pipelined. The order of V,F should be same for \\ both phases. \end{tabular} \\ %\\ 
\hline

& V\textsubscript{*} \{F\textsubscript{*} N\textsubscript{*}\}         & V\textsubscript{*} \{G\textsubscript{*}  F\textsubscript{*}\}        & \multicolumn{1}{c}\cmark     & \begin{tabular}[c]{@{}l@{}}Need support to connect \\agg and cmb units to\\ intermediate buffer\end{tabular}                                                             & \begin{tabular}[c]{@{}l@{}}HyGCN \cite{yan2020hygcn} \\ DAC GNN \cite{Auten2020} \\ (agg -\textgreater cmb)\end{tabular} & \begin{tabular}[c]{@{}l@{}} \textbf{Row(s) wise granularity}: Row(s) of intermediate \\ matrix indexed by V can be pipelined. The order \\ should not be (VFN,VFG) since that can be done \\ element wise. HyGCN allocates fixed number of \\ PEs per unit, which may lead to stalls. E.g., \\combination engine idle while waiting. HyGCN  \\ dataflow - $PP_{AC}(V_x F_s N_t, V_s G_s F_t)$\end{tabular} \\ %\\
\hline
& F\textsubscript{*} \{V\textsubscript{*} N\textsubscript{*}\}         & F\textsubscript{*} \{G\textsubscript{*}  V\textsubscript{*}\}        & \multicolumn{1}{c}\cmark     & \begin{tabular}[c]{@{}l@{}}Need support to connect \\agg and cmb units to\\ intermediate buffer\end{tabular}                                                            & \begin{tabular}[c]{@{}l@{}}(agg -\textgreater cmb)\end{tabular} & \begin{tabular}[c]{@{}l@{}} \textbf{Column(s) wise granularity}: Column(s) of the \\ intermediate matrix indexed by F can be \\ pipelined. The order should not be (FVN,FVG).\end{tabular} \\ %\\
\hline
  & \{N\textsubscript{*} F\textsubscript{*}\} V\textsubscript{*}         & \{V\textsubscript{*} G\textsubscript{*}\}  F\textsubscript{*}        & \multicolumn{1}{c}\cmark    & \begin{tabular}[c]{@{}l@{}}Need support to connect \\agg and cmb units to\\ intermediate buffer\end{tabular}                                                            & \begin{tabular}[c]{@{}l@{}}(cmb -\textgreater agg)\end{tabular} & \begin{tabular}[c]{@{}l@{}}\textbf{Element(s) wise granularity}: The order should \\be (NFV, VGF) or (FNV, GVF). V$\times$G matrix \\after cmb becomes N $\times$ F for agg. \end{tabular} \\ %\\
\hline
& N\textsubscript{*} \{V\textsubscript{*} F\textsubscript{*}\}         & V\textsubscript{*} \{G\textsubscript{*}  F\textsubscript{*}\}        & \multicolumn{1}{c}\cmark     & \begin{tabular}[c]{@{}l@{}}Need support to connect \\agg and cmb units to\\ intermediate buffer\end{tabular}                                                           & \begin{tabular}[c]{@{}l@{}} (cmb -\textgreater agg)\end{tabular} & \begin{tabular}[c]{@{}l@{}} \textbf{Row(s) wise granularity}: Order should not be \\(NFV, VGF) since it can be done element wise.\end{tabular} \\ %\\
\hline
& F\textsubscript{*} \{V\textsubscript{*} N\textsubscript{*}\}         & G\textsubscript{*} \{F\textsubscript{*}  V\textsubscript{*}\}        & \multicolumn{1}{c}\cmark     & \begin{tabular}[c]{@{}l@{}}Need support to connect \\agg and cmb units to\\ intermediate buffer\end{tabular}                                                             & \begin{tabular}[c]{@{}l@{}}AWB-GCN \cite{geng2019awb} \\ (cmb -\textgreater agg)\end{tabular} & \begin{tabular}[c]{@{}l@{}} \textbf{Column(s) wise granularity}: The order should \\ not be (FNV, GVF). AWB-GCN enables flexible \\ allocation of PEs for different phases to match \\ production and consumption rates. AWB-GCN  \\dataflow-
%$PP_{CA}(G_t F_t V_s, F_s N_t V_s)$ 
$PP_{CA}(F_s N_t V_s, G_t F_t V_s)$
\end{tabular}                                                                                                                           \tabularnewline \bottomrule                                              
\end{tabular}
\label{tables:interleave}
\vspace{-3mm}
\end{table*}

==> tables/interleave_bk.tex <==
\begin{table*}[]
\begin{tabular}{lllllll}
\textbf{Sequential}          & \{Vx, Fx, Nx\} & \{Vx, Gx, Fx\} & \begin{tabular}[c]{@{}l@{}}Buffer \& Data \\ Scheduler\end{tabular}                                                                            & \begin{tabular}[c]{@{}l@{}}NOC \& PEs requirement\\  depends on accelerator\end{tabular}                                                         & \begin{tabular}[c]{@{}l@{}}TPU, MAERI\\ (any direction)\end{tabular}                              & \begin{tabular}[c]{@{}l@{}}Similar to running one full or tiled layer at a time. Outputs of \\ one layer gets stored in S2 scratchpad / buffer and rescheduled\\ back into the PEs.\end{tabular}                                                                                                                                                                                                \\
\textbf{Sequential Pipeline} & \{Vs, Fs, Nt\} & \{Vs, Gs, Ft\} & \begin{tabular}[c]{@{}l@{}}None, output of one unit \\ is stationary in the PEs, \\ and can be used as input\\ for the next layer\end{tabular} & \begin{tabular}[c]{@{}l@{}}Requires in place\\ accumulation (so output \\ can be buffered inside PE\\ to use as inputs)\end{tabular}             & \begin{tabular}[c]{@{}l@{}}EnGN (comb --\textgreater agg)\\ (agg -\textgreater comb)\end{tabular} & \begin{tabular}[c]{@{}l@{}}Agg. uses Fs if it is agg --\textgreater comb, and Gs if it is comb --\textgreater agg.\\ Interleaved is possible because the output of combination (V,G) matrix is stationary, \\ and the input to agg is also (V, G), which is also stationary!\\ for agg-\textgreater{}comb, may need circular buffer to stream in property bank (might be temporal)\end{tabular} \\
                             & \{Vx, Fx, Nx\} & \{Vx, Gx, Fx\} & Buffer \& Data Scheduler                                                                                                                       & \begin{tabular}[c]{@{}l@{}}NoC must be able to transfer\\ data to the corresponding\\ PEs (need 2 compute engine\\ or allocate PEs)\end{tabular} &                                                                                                   & will be a buffer/ setup in between aggregation and combination                                                                                                                                                                                                                                                                                                                                  \\
\textbf{Pipeline parallel}   & Vt, \{Fs, Nt\} & \{Vs, Gs, Ft\} & \begin{tabular}[c]{@{}l@{}}Buffer \& Data \\ Scheduler\end{tabular}                                                                            & \begin{tabular}[c]{@{}l@{}}Agg \& Comb both require\\ in place accumulation. Comb\\ Engine requires Store \& \\ Fwd links\end{tabular}           & HyGCN (agg -\textgreater comb)                                                                    & \begin{tabular}[c]{@{}l@{}}Has 'aggregation buffer and coordinator' between aggregation \& combination unit. \\ Fixed number of PEs per unit may lead to stalls between units.\\ Ex: combination engine idle, waiting for aggregation to finish\end{tabular}                                                                                                                                    \\
                             & \{Vs, Ft, Ns\} & \{Vs, Gt, Fs\} & Buffer \& Data Scheduler                                                                                                                       & \begin{tabular}[c]{@{}l@{}}Multicast NoC required\\ between PEs.\end{tabular}                                                                    & AWB-GCN (both ways)                                                                               & \begin{tabular}[c]{@{}l@{}}Authors looked into intra and Inter Layer pipelining. There is also flexible allocation\\ of PEs for different layers to match production and consumption rates.\end{tabular}                                                                                                                                                                                        \\
                             & \{Vx, Fx, Nx\} & \{Vx, Gx, Fx\} & Buffer \& Data Scheduler                                                                                                                       & \begin{tabular}[c]{@{}l@{}}NoC must be able to transfer\\ data to the corresponding\\ PEs (need 2 compute engine\\ or allocate PEs)\end{tabular} &                                                                                                   & Different dataflow and mappings --\textgreater different production and consumption rates                                                                                                                                                                                                                                                                                                      
\end{tabular}
\label{tables:interleavebk}
\end{table*}

==> tables/new/dataflow.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table}[]
\centering
\caption{Reuse opportunities for GEMM dimensions. (Intra-phase dataflow) \TK{the goal of this table is nice but I think we could simplify it and make it similar to Table II. @Eric - put a new table in "intra-phase dataflow" sheet in our spreadsheet. Can you put that here?}} %\TK{@Eric - can we replace this / augment this with a figure simply showing a GEMM mapped over a simple 2D array in a WS manner and show multicast of MK matrix, and spatial reduction across K?}}
\vspace{-0.25cm}
\begin{tabular}{|l|l|l|}
\hline
\textbf{Dataflow} & \textbf{\begin{tabular}[c]{@{}l@{}}Implication of \\ Loop Order\end{tabular}}                                           & \textbf{\begin{tabular}[c]{@{}l@{}}Implication of \\ Spatial Dimensions\end{tabular}}                                                                     \\ \hline
\{Ms Ns\} Kt      & \begin{tabular}[c]{@{}l@{}}Output (MN) stationary,\\ Inputs (MK) and \\ Weights (KN) stream \\ every cycle\end{tabular} & \begin{tabular}[c]{@{}l@{}}Spatial multicast of \\ Inputs and Weights every\\ cycle. Temporal reduction\\ of partial sums within \\ each PE.\end{tabular} \\ \hline
\{Ns Ks\} Mt      & \begin{tabular}[c]{@{}l@{}}Weight (KN) stationary,\\ Input (MK) streams\\ every cycle\end{tabular}                      & \begin{tabular}[c]{@{}l@{}}Spatial multicast of \\ inputs every cycle. \\ Spatial reduction of partial \\ sums across PEs\end{tabular}                    \\ \hline
\{Ms Ks\} Nt      & \begin{tabular}[c]{@{}l@{}}Input (MK) stationary, \\ Weight (KN) streams \\ every cycle\end{tabular}                    & \begin{tabular}[c]{@{}l@{}}Spatial multicast of \\ weights every cycle. \\ Spatial reduction of partial \\ sums across PEs\end{tabular}                   \\ \hline
\end{tabular}
\label{tables:dataflow}
\end{table}

==> tables/new/dataflow_bk.tex <==
% Please add the following required packages to your document preamble:
% \usepackage{multirow}
\begin{table*}[]
\centering
\caption{Reuse opportunities for GEMM dimensions. (Intra-phase dataflow) \TK{the goal of this table is nice but I think we could simplify it and make it similar to Table II. @Eric - put a new table in "intra-phase dataflow" sheet in our spreadsheet. Can you put that here?}} %\TK{@Eric - can we replace this / augment this with a figure simply showing a GEMM mapped over a simple 2D array in a WS manner and show multicast of MK matrix, and spatial reduction across K?}}
\vspace{-0.25cm}
\begin{tabular}{|l|l|l|l|l|l|l|l|l|l|l|l|l|l|}
\hline
\multicolumn{7}{|c|}{\textbf{Spatial}}                                                                                                                                                    & \multicolumn{7}{c|}{\textbf{Temporal}}                                                                              \\ \hline
\multirow{2}{*}{\textbf{Dimension}} & \multicolumn{3}{c|}{\textbf{Coupling}}                       & \multicolumn{3}{c|}{\textbf{Reuse}}                                                  & \multirow{2}{*}{\textbf{Dimension}} & \multicolumn{3}{c|}{\textbf{Coupling}} & \multicolumn{3}{c|}{\textbf{Reuse}}  \\ \cline{2-7} \cline{9-14} 
                                    & \textbf{B}         & \textbf{A}         & \textbf{O}         & \textbf{B}                 & \textbf{A}                 & \textbf{O}                 &                                     & \textbf{B}  & \textbf{A}  & \textbf{O} & \textbf{B} & \textbf{A} & \textbf{O} \\ \hline
\multirow{2}{*}{\textbf{M}}         & \multirow{2}{*}{}  & \multirow{2}{*}{Y} & \multirow{2}{*}{Y} & \multirow{2}{*}{Multicast} & \multirow{2}{*}{}          & \multirow{2}{*}{}          & K                                   & Y           & Y           &            &            &            & Reduction  \\ \cline{8-14} 
                                    &                    &                    &                    &                            &                            &                            & N                                   & Y           &             & Y          &            & Multicast  &            \\ \hline
\multirow{2}{*}{K}                  & \multirow{2}{*}{Y} & \multirow{2}{*}{Y} & \multirow{2}{*}{}  & \multirow{2}{*}{}          & \multirow{2}{*}{}          & \multirow{2}{*}{Reduction} & M                                   &             & Y           & Y          & Multicast  &            &            \\ \cline{8-14} 
                                    &                    &                    &                    &                            &                            &                            & N                                   & Y           &             & Y          &            & Multicast  &            \\ \hline
\multirow{2}{*}{N}                  & \multirow{2}{*}{Y} & \multirow{2}{*}{}  & \multirow{2}{*}{Y} & \multirow{2}{*}{}          & \multirow{2}{*}{Multicast} & \multirow{2}{*}{}          & M                                   &             & Y           & Y          & Multicast  &            &            \\ \cline{8-14} 
                                    &                    &                    &                    &                            &                            &                            & K                                   & Y           & Y           &            &            &            & Reduction  \\ \hline
\end{tabular}
\label{tables:dataflow}
\end{table*}

==> tables/new/inter-eqn-ea.tex <==
%\begin{scriptsize}
\begin{table}[t!]
\scriptsize
\vspace{-0.4cm}
  \centering
  \caption{Runtime and buffering requirements for Dataflows} %\SA{Is $PPel$ supposed to be written in subscript font?}\Rav{By PPel subscript I just meant that this is sum(max()) across all iterations of pipelining}}%\Rav{There is space for remarks too if needed}}
  %\TK{@Raveesh - by x do you mean you can do either s or t for that dimension? So does that mean each row is actually multiple datapoints? Thats confusing.}\Rav{It means that the datapoint that we choose for evaluation of that dataflow can have varaible tile sizes for dimension marked by X. S and T on the other hand mean that its NECESSARILY spatial or temporal}}
  \vspace{-0.25cm}
  \label{tables:inter_eq}
  \begin{tabular}{|l|l|l|}
    \hline
    \textbf{Inter-phase dataflow} & \textbf{Intermediate Buffering} & \textbf{Runtime}  \\
    
    \hline
    %Seq & $V\times F$ & $t_{AGG}+t_{CMB}$\\
    %\hline
    Seq & V$\times$F & t\textsubscript{AGG}+t\textsubscript{CMB}\\
    \hline
    SP-Generic & $PPel$ & t\textsubscript{AGG}+t\textsubscript{CMB}\\
    \hline
    %SP-EnGN-like & $0$ & $t_{AGG}+t_{CMB}-t_{load}$\\
    %\hline
    SP-Optimized & 0 & t\textsubscript{AGG}+t\textsubscript{CMB}-t\textsubscript{load}\\
    \hline
    %PP-Element & $2\times T\_V\times T\_F$ & \\
    %\hline
   PP & 2$\times PPel$ & sum(max(t\textsubscript{AGG},t\textsubscript{CMB})\textsubscript{PPel})\\
    \hline
  \end{tabular}
\vspace{-2mm}
\end{table}
%\end{scriptsize}

==> tables/new/interleave_bk.tex <==
\begin{table*}[]
\begin{tabular}{lllllll}
\vspace{-0.25cm}
\textbf{Sequential}          & \{Vx, Fx, Nx\} & \{Vx, Gx, Fx\} & \begin{tabular}[c]{@{}l@{}}Buffer \& Data \\ Scheduler\end{tabular}                                                                            & \begin{tabular}[c]{@{}l@{}}NOC \& PEs requirement\\  depends on accelerator\end{tabular}                                                         & \begin{tabular}[c]{@{}l@{}}TPU, MAERI\\ (any direction)\end{tabular}                              & \begin{tabular}[c]{@{}l@{}}Similar to running one full or tiled layer at a time. Outputs of \\ one layer gets stored in S2 scratchpad / buffer and rescheduled\\ back into the PEs.\end{tabular}                                                                                                                                                                                                \\
\textbf{Sequential Pipeline} & \{Vs, Fs, Nt\} & \{Vs, Gs, Ft\} & \begin{tabular}[c]{@{}l@{}}None, output of one unit \\ is stationary in the PEs, \\ and can be used as input\\ for the next layer\end{tabular} & \begin{tabular}[c]{@{}l@{}}Requires in place\\ accumulation (so output \\ can be buffered inside PE\\ to use as inputs)\end{tabular}             & \begin{tabular}[c]{@{}l@{}}EnGN (comb --\textgreater agg)\\ (agg -\textgreater comb)\end{tabular} & \begin{tabular}[c]{@{}l@{}}Agg. uses Fs if it is agg --\textgreater comb, and Gs if it is comb --\textgreater agg.\\ Interleaved is possible because the output of combination (V,G) matrix is stationary, \\ and the input to agg is also (V, G), which is also stationary!\\ for agg-\textgreater{}comb, may need circular buffer to stream in property bank (might be temporal)\end{tabular} \\
                             & \{Vx, Fx, Nx\} & \{Vx, Gx, Fx\} & Buffer \& Data Scheduler                                                                                                                       & \begin{tabular}[c]{@{}l@{}}NoC must be able to transfer\\ data to the corresponding\\ PEs (need 2 compute engine\\ or allocate PEs)\end{tabular} &                                                                                                   & will be a buffer/ setup in between aggregation and combination                                                                                                                                                                                                                                                                                                                                  \\
\textbf{Pipeline parallel}   & Vt, \{Fs, Nt\} & \{Vs, Gs, Ft\} & \begin{tabular}[c]{@{}l@{}}Buffer \& Data \\ Scheduler\end{tabular}                                                                            & \begin{tabular}[c]{@{}l@{}}Agg \& Comb both require\\ in place accumulation. Comb\\ Engine requires Store \& \\ Fwd links\end{tabular}           & HyGCN (agg -\textgreater comb)                                                                    & \begin{tabular}[c]{@{}l@{}}Has 'aggregation buffer and coordinator' between aggregation \& combination unit. \\ Fixed number of PEs per unit may lead to stalls between units.\\ Ex: combination engine idle, waiting for aggregation to finish\end{tabular}                                                                                                                                    \\
                             & \{Vs, Ft, Ns\} & \{Vs, Gt, Fs\} & Buffer \& Data Scheduler                                                                                                                       & \begin{tabular}[c]{@{}l@{}}Multicast NoC required\\ between PEs.\end{tabular}                                                                    & AWB-GCN (both ways)                                                                               & \begin{tabular}[c]{@{}l@{}}Authors looked into intra and Inter Layer pipelining. There is also flexible allocation\\ of PEs for different layers to match production and consumption rates.\end{tabular}                                                                                                                                                                                        \\
                             & \{Vx, Fx, Nx\} & \{Vx, Gx, Fx\} & Buffer \& Data Scheduler                                                                                                                       & \begin{tabular}[c]{@{}l@{}}NoC must be able to transfer\\ data to the corresponding\\ PEs (need 2 compute engine\\ or allocate PEs)\end{tabular} &                                                                                                   & Different dataflow and mappings --\textgreater different production and consumption rates                                                                                                                                                                                                                                                                                                      
\end{tabular}
\label{tables:interleavebk}
\end{table*}

==> tables/new/related.tex <==
%\begin{scriptsize}
\begin{table}[!t]
\scriptsize
\vspace{-0.4cm}
  \centering
  \caption{Features and capabilities of dataflow studies} %\SA{Is $PPel$ supposed to be written in subscript font?}\Rav{By PPel subscript I just meant that this is sum(max()) across all iterations of pipelining}}%\Rav{There is space for remarks too if needed}}
  %\TK{@Raveesh - by x do you mean you can do either s or t for that dimension? So does that mean each row is actually multiple datapoints? Thats confusing.}\Rav{It means that the datapoint that we choose for evaluation of that dataflow can have varaible tile sizes for dimension marked by X. S and T on the other hand mean that its NECESSARILY spatial or temporal}}
  \vspace{-0.25cm}
  \label{tables:related}
  \begin{tabular}{|l|l|l|l|l|}
    \hline
    \textit{Studies} & \textit{Tools} & \textit{Dense} & \textit{Sparse} & \textit{Multi-} \\
    & & & & \textit{phase}\\
    \hline
    Kwon et al~\cite{kwon2019understanding} & MAESTRO & \cmark & \xmark &\xmark \\
    \hline
     Eyeriss~\cite{eyeriss2016isca} & Custom RTL & \cmark & \xmark &\xmark \\
    \hline
     Parashar et al~\cite{timeloop} & Timeloop & \cmark & \xmark &\xmark \\
    \hline
     Interstellar~\cite{interstellar} & Halide toolflow & \cmark & \xmark &\xmark \\
    \hline
     This work & STONNE~\cite{stonnecal} & \cmark & \cmark &\cmark \\
    \hline
  \end{tabular}
\vspace{-1mm}
\end{table}
%\end{scriptsize}

==> tables/new/workload_cat.tex <==
\begin{table}[ht!]
\footnotesize
  \centering
  \caption{Different categories of workloads.}
  \vspace{-0.25cm}
  \label{tables:workload_cat}
  \begin{tabular}{|l|l|l|}
    \hline
    \textbf{Category} & \textbf{Description} & \textbf{Workloads}  \\
    \hline
    Category 1 & Denser graphs (high edges & Collab, Imdb\\
    & per vertex) and low features & \\ 
    %& and low features &\\
    \hline
    Category 2 & High input features (F) & RedditBIN, Citeseer, Cora \\
    \hline
    Category 3 & Sparser graphs and & Proteins, Mutag \\
    &  low input features &\\
    \hline
  \end{tabular}
\end{table}


==> tables/workload.tex <==
\begin{footnotesize}


\begin{table}[ht!]
  \centering
  \caption{Datasets information. First half for graph classification (we use batch size of 64), bottom half for node classification. (* means that indicator vectors were used in place of features).}
  \label{tables:workload}
\begin{tabular}{lllll}
\toprule
\textbf{Name}   & \textbf{\#Graphs} & \textbf{\begin{tabular}[c]{@{}l@{}}\#Nodes \\ (avg)\end{tabular}} & \textbf{\begin{tabular}[c]{@{}l@{}}\#Edges \\ (avg)\end{tabular}} & \textbf{\#Features} \\
\toprule
Mutag% (MU)
& 188                & 17.93                                                              & 19.79                                                              & 28*                  \\
Proteins% (PR)
& 1113               & 39.06                                                              & 72.82                                                              & %1(reg)/
29(full)                   \\
Imdb-bin% (IB)
& 1000               & 19.77                                                              & 96.53                                                              & 136*                 \\
Reddit-bin% (RB)
& 2000               & 429.63                                                             & 497.75                                                             & 3782*                \\
Collab% (CL)
& 5000               & 74.49                                                              & 2457.78                                                            & 492*                 \\
\hline
%Pubmed (PB)     & 1                  & 19,717                                                             & 88,676                                                             & 500                  \\
Citeseer% (CS)
& 1                  & 3327                                                               & 9464                                                               & 3703                 \\
Cora% (CR)
& 1                  & 2708                                                               & 10858                                                              & 1433                 \\
%Reddit (RE)     & 1                  & 232,965                                                            & 114,615,892                                                        & 602   \tabularnewline

\bottomrule
\end{tabular}
\vspace{-3mm}
\end{table}
\end{footnotesize}

==> tables/workload_cat.tex <==
\begin{scriptsize}
\begin{table}[ht!]
  \centering
  \caption{Different categories of workloads.}
  \label{tables:workload_cat}
  \begin{tabular}{|l|l|l|}
    \hline
    \textbf{Category} & \textbf{Description} & \textbf{Workloads}  \\
    \hline
    Category 1 & Denser graphs & Collab, Imdb\\
    & (High edges per vertex) & \\ & and low features &\\
    \hline
    Category 2 & High input features (F) & RedditBIN,Citeseer,Cora \\
    \hline
    Category 3 & Sparser graphs and & Proteins, Mutag \\
    &  low input features &\\
    \hline
  \end{tabular}
\vspace{-3mm}
\end{table}
\end{scriptsize}
